Adaptive Sampling of Latent Phenomena using Heterogeneous Robot Teams (ASLaP-HR)

In this paper, we present an online adaptive planning strategy for a team of robots with heterogeneous sensors to sample from a latent spatial field using a learned model for decision making. Current robotic sampling methods seek to gather information about an observable spatial field. However, many applications, such as environmental monitoring and precision agriculture, involve phenomena that are not directly observable or are costly to measure, called latent phenomena. In our approach, we seek to reason about the latent phenomenon in real-time by effectively sampling the observable spatial fields using a team of robots with heterogeneous sensors, where each robot has a distinct sensor to measure a different observable field. The information gain is estimated using a learned model that maps from the observable spatial fields to the latent phenomenon. This model captures aleatoric uncertainty in the relationship to allow for information theoretic measures. Additionally, we explicitly consider the correlations among the observable spatial fields, capturing the relationship between sensor types whose observations are not independent. We show it is possible to learn these correlations, and investigate the impact of the learned correlation models on the performance of our sampling approach. Through our qualitative and quantitative results, we illustrate that empirically learned correlations improve the overall sampling efficiency of the team. We simulate our approach using a data set of sensor measurements collected on Lac Hertel, in Quebec, which we make publicly available.

==> 02_Preliminaries.tex <==
\subsection{Related Work.}
There are myriad problem spaces that involve planning the path of mobile sensors. Bayesian optimization approaches seek to find the maximum of a spatial field \cite{marchant_sequential_2014, ott_bayesian_2019, tan_gaussian_2018}; exploration and active mapping optimize the observation of an unknown area \cite{yamauchi_frontier-based_1998, lluvia_active_2021, vidal-calleja_informative_2020}; and active information gathering or target tracking focuses on estimating the state of dynamic hidden states \cite{tzes_technical_2021,kantaros_sampling-based_2021,salam_adaptive_2019}. Although there are many objective functions studied among these applications, which can be categorized as information-theoretic \cite{nieto_coordinating_2019}, such as mutual information \cite{low_information-theoretic_2009, singh_efficient_2009}, and not information-driven, as is the case in hotspot sampling \cite{low_adaptive_2008, manjanna_policy_2020}. This work seeks to maximize the expected information gained by the robot team; thus, we categorize our work as adaptive informative sampling (or informative path planning).

In addition to the objective, adaptive informative sampling problems can vary in many dimensions, from the time horizons of planning to the types of action and motion uncertainty considered. The novel problem formulation that we present in Section~\ref{Sec:Problem} is not restricted to myopic or non-myopic approaches, nor does it restrict the consideration of motion uncertainty and arbitrary set of actions,\footnote{The problem formulation considers a discrete action set. Using continuous dynamics would require slight reformulation} though the methods presented in Section~\ref{Sec:Approach} are myopic and do not consider motion uncertainty. For a broader discussion of the many dimensions of information-driven path planning, see the survey by Bai~\etal \cite{liu_information-driven_2021}. The core aspects of the adaptive informative sampling problem investigated in this paper are heterogeneous multi-robot teams and planning in a latent spatial field.

Heterogeneity of multi-robot teams can vary drastically. Manjanna~\etal use two autonomous surface vehicles, one with a water quality sensor and the other with a water sampler, where the sensor vehicle explores to inform the samplers decision \cite{manjanna_heterogeneous_2018}. Similarly, Manderson~\etal use an aerial vehicle to inform the decisions of a ground vehicle \cite{manderson_heterogeneous_2019}. Chand and Carnegie investigated heterogeneous processing and sensing capabilities to assign tasks to different robot types, where robots with low-value sensing do computation rather than exploration tasks \cite{chand_mapping_2013}. Shi~\etal use a Voronoi approach where the space is partitioned according to heterogeneous capabilities, like mobility constraints in ground versus aerial vehicles \cite{shi_adaptive_2020}. Similarly, Cai~\etal consider heterogeneous capabilities such as field of view and traversability of different types of environment \cite{cai_non_2021}. Whereas Chand and Carnegie model different levels of sensing ability (e.g., low vs high), we model qualitatively different sensor types, which all take high quality sensor measurements in their respective observable space. Manjanna~\etal and Manderson~\etal investigate different robot types (sensor vs sampler, and aerial vs ground sensing, respectively), but their investigations focus on two types with prescribed roles. We model an arbitrary number of sensor types where tasks and roles are not predesigned.

Recent work has only just begun to develop models and algorithms to make real-time decisions with respect to a latent phenomenon of interest. Arora~\etal study multi-modal active perception, where measurements must be combined with domain knowledge to deduce information about variables or phenomena that cannot be directly measured \cite{arora_multi-modal_2019}. Their paper investigates a single robot with multiple sensors that make discrete observations and maps the observations to the variables of interest through an expert designed Bayesian network. In this work, we consider a multi-robot team where sensor measurements are continuous and we learn a continuous representation mapping from the observations to the latent phenomenon of interest. 

\subsection{Contributions} We formalize adaptive informative sampling for multiple continuous sensors to maximize information theoretic objective of a latent phenomenon. We use a robot team with heterogeneous sensor types to measure observable spatial fields. A learned model from historical data enables the robot team to make inferences about the latent spatial field in real time and use these inferences to choose sample locations that maximize the information gain of the latent phenomenon. Additionally, we learn correlations \textbf{among} the multiple observable spatial fields; these correlations are learned offline and are used to make real-time decisions regarding sampling locations. We investigate the impact of the learned correlations, demonstrating the improvement in sampling through simulation of a myopic planning algorithm. Our main contributions are:
\begin{itemize}
    \item We formulate the ASLaP problem as the maximization of the expected information of a latent spatial field. 
    \item We develop ASLaP-HR, an adaptive sampling approach for a team of robots with heterogeneous sensors using a learned mapping from observations to the latent phenomenon.
    \item We show that the learned correlations among the observable spatial fields improve the sampling efficiency of our adaptive sampling approach.
\end{itemize} 

We simulate two sets of experiments, one with synthetic data and the other using sensor measurements collected on a lake. The sensor data, which we make publicly available \footnote{This data is available at: \url{https://github.com/SandeepManjanna/water_quality_dataset}}, includes co-located measurements of ten sensors; our experiments use three of the ten sensor fields, two as the sensor spaces and one as the latent variable of interest. The simulations show that learned correlations among the observable spatial fields improve sampling; qualitatively, the team naturally spread out their measurements, and quantitatively, the mean squared error of the latent spatial field estimate is lower when using the learned correlations. Future work will investigate the online learning of these relationships.

==> snippets/30_fig_intro.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics[width = 0.975\columnwidth]{figures/ag_concept.pdf}
    \caption{System overview depicting two robots with unique sensor types, one measuring the red spatial field the other measuring the blue spatial field. Together, they seek information about an underlying latent phenomenon.}
    \label{fig:proxies}
    %\vspace{-0.3cm}
\end{figure}

==> snippets/32_fig_frontier.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics[width = 0.9\columnwidth]{figures/empty.eps}
    \caption{8 grid points for considering next move.}
    \label{fig:frontier}
    %\vspace{-0.3cm}
\end{figure}

==> snippets/37_fig_time2completion.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics[width = 0.8\columnwidth]{figures/completion_time.pdf}
    \caption{\fix{add}}
    \label{fig:time2completion}
    %\vspace{-0.3cm}
\end{figure}

==> snippets/38_fig_example.tex <==
\begin{figure*}[tb]
  \begin{subfigure}{0.26\textwidth}
    \centering
    \includegraphics[width = \columnwidth]{figures/example_rawdata.pdf}
    \caption{Historical Data} \label{fig:example-data}
  \end{subfigure}
  \begin{subfigure}{0.74\textwidth}
    \centering
    \includegraphics[width = 0.3\columnwidth]{figures/example0.pdf}
    \includegraphics[width = 0.3\columnwidth]{figures/example1.pdf}
    \includegraphics[width = 0.3\columnwidth]{figures/example2.pdf}
    \caption{Spatial fields.} \label{fig:example-fields}
  \end{subfigure}%
%   \hspace*{\fill}   % maximizeseparation between the subfigures
    \caption{\edit{Visual representation of Example~\ref{ex:ag}. \textit{(a)} Historical data is used to train a machine learning model that take sensor measurements (chlorophyll and soil conductivity) as input and predict nutrient level. \textit{(b)} Knowing the spatial field of nutrient levels is most helpful to a farmer, but it requires time-consuming leaf samples. Instead, a team of robots measure chlorophyll and soil conductivity and use the machine learning model from (a) to make real-time decisions about where sensor measurements most inform the estimate of nutrition.} }
    \label{fig:example}
\end{figure*}

==> snippets/38_fig_example2.tex <==
\begin{figure*}[tb]
  \begin{subfigure}{0.23\textwidth}
    \centering
    \includegraphics[width = \columnwidth]{figures/example_rawdata.pdf}
    \caption{Historical Data} \label{fig:example-data}
  \end{subfigure}%\hspace{-1em}
  \begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width = 0.32\columnwidth]{figures/example_tall0.pdf}
    \includegraphics[width = 0.32\columnwidth]{figures/example_tall1.pdf}
    \includegraphics[width = 0.32\columnwidth]{figures/example_tall2.pdf}
    \caption{Spatial fields.} \label{fig:example-fields}
  \end{subfigure}%\hspace{-1em}%
  \begin{subfigure}{0.24\textwidth}
    \centering
    \includegraphics[width = \columnwidth]{figures/ag_concept.pdf}
    \caption{Multi-robot information gathering.} \label{fig:example-fields}
  \end{subfigure}%
%   \hspace*{\fill}   % maximizeseparation between the subfigures
    \caption{Visual representation of Example~\ref{ex:ag}. \textit{(a)} Historical data is used to train a machine learning model to predict nutrient levels from chlorophyll and soil conductivity measurements. \textit{(b)} Farms can be described by various spatial fields. The nutrient level spatial field is most informative to a farmer, but it requires costly and time-consuming leaf samples. Chlorophyll and soil conductivity spatial fields can be measured quickly and cheaply by sensors. \textit{(c)} A team of robots can measure chlorophyll and soil conductivity relatively efficiently and use the learned model from (a) to make real-time decisions about where \edit{to sample and which} sensor measurements most inform the estimate of nutrition.}
    \label{fig:example}
\end{figure*}
